Modeling COVID-19 optimal testing strategies in long-term care facilities: An optimization-based approach

Long-term care facilities have been widely affected by the COVID-19 pandemic. Retirement homes are particularly vulnerable due to the higher mortality risk of infected elderly individuals. Once an outbreak occurs, suppressing the spread of the virus in retirement homes is challenging because the residents are in contact with each other, and isolation measures cannot be widely enforced. Regular testing strategies, on the other hand, have been shown to effectively prevent outbreaks in retirement homes. However, high frequency testing may consume substantial staff working time, which results in a trade-off between the time invested in testing, and the time spent providing essential care to residents. Thus, developing an optimal testing strategy is crucial to proactively detect infections while guaranteeing efficient use of limited staff time in these facilities. Although numerous efforts have been made to prevent the virus from spreading in long-term care facilities, this is the first study to develop testing strategies based on formal optimization methods. This paper proposes two novel optimization models for testing schedules. The models aim to minimize the risk of infection in retirement homes, considering the trade-off between the probability of infection and staff workload. We employ a probabilistic approach in conjunction with the optimization models, to compute the risk of infection, including contact rates, incidence status, and the probability of infection of the residents. To solve the models, we propose an enhanced local search algorithm by leveraging the symmetry property of the optimal solution. We perform several experiments with realistically sized instances and show that the proposed approach can derive optimal testing strategies.

==> draft.tex <==
\textbf{Covid-19 pandemic in LTCFs} 

LTCFs include institutions such as nursing homes, retirement homes, rehabilitation homes, and other facilities that provide medical and personal support to patients, usually older age groups \cite{danis2020high}. These organizations aim to provide high-quality care for the elderly population at a lower cost.


LTCFs have been widely affected by the COVID-19 pandemic \cite{gmehlin2020covid, giri2021nursing}. This is because of the high density of elderly residents at high risk for morbidity and mortality by being infected with COVID-19. In addition, the residents, in most cases, have pre-existing conditions (i.e., diabetes, respiratory disease, hypertension, chronic heart diseases), which makes the diagnosis of the virus difficult \cite{childs2019burden, moyo2020risk}. 

Besides the factors related to the residents, other aspects have been reported as the main causes of outbreaks in LTCFs, among them, understaffing, residents sharing common spaces, and the high contact with the staff \cite{gorges2020staffing, giri2021nursing, chen2021nursing}. Several IPC recommendations have been considered in LTCFs to mitigate the spread of the virus, such as social distancing, daily screening (testing) of staff and residents, isolation, and visitation restrictions. In Germany, \cite{german2021bulletin} studied the COVID-19 outbreaks in nursing homes and found that symptom control and testing, vaccination, and reduction of the national incidence are effective prevention strategies. Cohort isolation of positive residents in conjunction with widespread screening has also been considered as a strategy to prevent the spread of the virus \cite{krone2021control}. 
% for containing the spread of the virus
 
%Testing strategy importance
Despite the recommendations from the health authorities to mitigate the spread of COVID-19, LTCFs are still at risk of outbreaks. Asymptomatic transmission among the residents and staff was found as one of the main causes of virus spread, and mortality \cite{birgand2021testing, roxby2020outbreak, giri2021nursing, borras2020asymptomatic}. \cite{roxby2020outbreak} performed an outbreak investigation in a nursing home in Seattle; It was found that symptom screening fails to identify infected residents. In contrast, preventive testing combined with safety strategies can reduce viral spread. Similarly, \cite{telford2020preventing}, and \cite{graham2020sars} demonstrated that facility wide-testing is an efficient strategy to prevent COVID-19 outbreaks since it helps to identify asymptomatic infections in LTCFs proactively. Overall, widespread testing in LTCFs has shown to be one of the most efficient strategies to contain outbreaks. The proactive testing strategy combined with other protocols, such as isolation and quarantine, facilitates the timely implementation of control procedures due to the early detection of the virus \cite{kucharski2020effectiveness, bergstrom2020frequency}.  



\iffalse



%Residents in Long-Term Care Facilities (LTCF), such as Retirement Homes (RH), nursing homes, and rehabilitation facilities, have been highly affected by the coronavirus disease 2019 (COVID-19) pandemic \cite{jordan2020covid, onder2020case}. These organizations provide medical and personal support to patients, usually older age groups \cite{danis2020high}. 




The elderly population in these institutions are at a significantly higher risk of contracting the severe acute respiratory syndrome coronavirus (SARS-CoV-2) (hereafter COVID-19) . 




%%With numbers
The residents in LTCFs, particularly in RHs, are in regular contact with each other and the staff. Thus, controlling the spreading of the pandemic by isolating the residents is a challenge \cite{danis2020high}.





have been highly affected by the coronavirus disease 2019 (COVID-19) pandemic . LTCFs include institutions such as nursing homes, Retirement Homes (RH), rehabilitation
facilities, and other facilities that provide medical and personal support to patients, usually older age groups \cite{danis2020high}. 

%%Why they are vulnerable%% how is the spread
LTCFs have been widely affected by the COVID-19 pandemic \cite{gmehlin2020covid, giri2021nursing}. This is because of the high density of elderly residents at high risk for morbidity and mortality by being infected with COVID-19. In addition, the residents, in most cases, have pre-existing conditions (i.e., diabetes, respiratory disease, hypertension, chronic heart diseases), which makes the diagnosis of the virus difficult \cite{childs2019burden, moyo2020risk}. 

\fi


